Concise Read-Only Specifications for Better Synthesis of Programs with Pointers -- Extended Version

In program synthesis there is a well-known trade-off between concise and strong specifications: if a specification is too verbose, it might be harder to write than the program; if it is too weak, the synthesised program might not match the user's intent. In this work we explore the use of annotations for restricting memory access permissions in program synthesis, and show that they can make specifications much stronger while remaining surprisingly concise. Specifically, we enhance Synthetic Separation Logic (SSL), a framework for synthesis of heap-manipulating programs, with the logical mechanism of read-only borrows. We observe that this minimalistic and conservative SSL extension benefits the synthesis in several ways, making it more (a) expressive (stronger correctness guarantees are achieved with a modest annotation overhead), (b) effective (it produces more concise and easier-to-read programs), (c) efficient (faster synthesis), and (d) robust (synthesis efficiency is less affected by the choice of the search heuristic). We explain the intuition and provide formal treatment for read-only borrows. We substantiate the claims (a)--(d) by describing our quantitative evaluation of the borrowing-aware synthesis implementation on a series of standard benchmark specifications for various heap-manipulating programs.

==> Makefile <==
all: Makefile *.tex *.bib
	pdflatex --jobname=paper paper
	bibtex paper -min-crossrefs=5
	pdflatex --jobname=paper paper
	pdflatex --jobname=paper paper

ext:
	pdflatex --jobname=paper-extended "\def\extflag{}\input{paper}"
	bibtex paper-extended -min-crossrefs=5
	pdflatex --jobname=paper-extended "\def\extflag{}\input{paper}"
	pdflatex --jobname=paper-extended "\def\extflag{}\input{paper}"


clean:
	rm -f *.aux *.bbl *.blg *.log *.out *.rel paper.pdf paper.zip	

.PHONY: all clean

zip:
	zip paper.zip Makefile *.tex *.bbl mathpartir.sty references.bib frameit.sty llncs.cls fig/*.tex fig/*.pdf tables/*


==> algorithm.tex <==

\section{Modified Synthesis Algorithm}
\label{sec:modif-synth-algor}

\is{Discuss how the new rules should be positioned in the algorithm:}

\begin{itemize}
\item Which phase should the rule be added? Give an example of what goes wrong if positioned at a wrong place.
\item Any specific optimisations they enable?
\end{itemize}


==> aux_corollary.tex <==
\begin{corollary}[Borrows Always Return]
  \label{cr:borrows}
  Given 
  \mcode{\ctx,\fun; \env;
    \trans
    {\asn{\phi;P}}
    {\asn{\slQ}}
    {\prog}
  } for a goal named \mcode{f},
  taking 
  \mcode{\fun \eqdef f(\many{x_i}) :
    \asn{\phi_f;P_f}
    {\asn{\slQ_f}}}
  with well-formed specifications, and leading to
  \mcode{\ctx,\fun; \env;
    \trans
    {\asn{\phi';P'}}
    {\asn{\slQ}}
    {f(\many{y_i});\prog}
  }
  for a substitution \mcode{\subst}, if:
  \begin{enumerate}[label=\emph{(\roman*)}]
  \item 
    \mcode{P   = \iblock{y}{n}{{\iiann}} \sep R}
    and
    \mcode{P_f = \iblock{x}{m}{{\ann}} \sep R_f}
    and
    \mcode{\phi_f \centernot\implies (\ann = \mut)}
    and
    \mcode{\subst=[\subst',\subs{x}{y},\subs{\ann}{\iiann}]}
    then 
    \mcode{P'  = \iblock{y}{n}{{\iiann}} \sep R'}.
  \item 
    \mcode{P   = \ispointsto{y}{e}{{\iiann}} \sep R}
    and
    \mcode{P_f = \ispointsto{x}{e_f}{{\ann}} \sep R_f}
    and
    \mcode{\phi_f \centernot\implies (\ann = \mut)}
    and
    \mcode{\subst=[\subst',\subs{x}{y},\subs{\ann}{\iiann}]}
    then either
    \mcode{P'  = \ispointsto{y}{e}{{\iiann}} \sep R'} or
    \mcode{f} deallocates the heap  pointed by \mcode{y}.
  \item 
    \mcode{P   = \ipred{p}{\many{e_i}}{} \sep R}
    and
    \mcode{P_f = \ipred{p}{\many{e'_i}}{} \sep R_f}
    and
    \mcode{i \in 1..n}
    then either
    \mcode{P'  =  \ipred{p}{\many{e''_i}}{} \sep R'}
    where
    \mcode{\forall i \in 1..n,
      (\phi_f \centernot\implies e'_i =\mut)
      \implies
      e_i =  e''_i
    }
    or
    \mcode{f} deallocates the heap described by
    \mcode{\ipred{p}{\many{e_i}}{}}.
  \end{enumerate}
\end{corollary}


==> auxiliary_proofs-2.tex <==
\section*{Syntax}

See \autoref{fig:lang} for the programming language and \autoref{fig:logic} for the assertion language.
%
For simplicity, we formalize a core language without theories;
the only sorts in the core language are locations, booleans, and permissions
(where permissions appear only in specifications)
and the pure logic only has equality.
%
In contrast, our implementation supports integers and sets
(where the latter also only appear in specifications),
with linear arithmetic and standard set operations.
%
Although we do not formalize sort-checking of formulae,
for readability, we will use the meta-variable $\alpha$ where the intended sort of the pure logic term is ``permission''. 
%
\np{I also relaxed syntactic restrictions on blocks and predicate instances
  that required their subformulas to be variables. I think it was an
  unnecessary restriction, but feel free to change it back if it breaks
  anything.}
\ac{i wondered the same at some point. It doesn't break anything. We can
  leave it like this.}


\begin{figure}[t]
\setlength{\belowcaptionskip}{-10pt}
%\setlength{\abovecaptionskip}{-10pt}
\centering
\[
\!\!\!\!
{\small
\begin{array}{l@{\!\!}r@{\ \ }c@{\ \ }l}
  \text{Variable} & x, y & & \text{Alpha-numeric identifiers}
  \\[2pt]
  \text{Expression} & e & ::= &
   0 \mid \True \mid x \mid e = e \mid e \wedge e \mid \neg e
  \qquad \qquad \quad
  \text{Size, offset}   ~~ \size, \off \qquad \text{Non-negative integers}
  \\[2pt]
  % \text{Expression} & e & ::= &
   % d \mid x \mid e = e \mid e \wedge e \mid \neg e
  % \\[2pt]
  \text{Command} &
  c & ::= &
            \Letz~{x} = \deref{(x + \off)} \mid
            \deref{(x + \off)} = e \mid 
            \Letz~{x} = \malloc{\size} \mid
            \free{x} \\
            & & & \mid \cerror \mid f(\many{e_i})
            \mid c; c \mid % \cmagic \mid
        \Ifz (e) \set{c}~\Elsez \set{c}
  % \\[2pt]
  % \text{Type} & t & ::= &
  % \typ{loc} \mid \typ{int} \mid \typ{bool} \mid \typ{set}
  % \\[2pt]
  % \text{Function} & \fundef & ::= & f~(\many{t_i~x_i})~\set{~c~}
  \\[2pt]
  % \text{Fun. dict.} & \fctx & ::= & \epsilon \mid \fctx, f~(\many{t_i~x_i})~\set{~c~}
  \text{Fun. dict.} & \fctx & ::= & \epsilon \mid \fctx, f~(\many{x_i})~\set{~c~}
\end{array}
}
\]
\caption{Programming language grammar.}
\label{fig:lang}
\end{figure}


\begin{figure}[t]
  \centering
%
\[
\!\!\!\!\!\!\!\!\!\!\!\!
{\small
\begin{array}{l@{\ \ }l@{\ \ }c@{\ \ }l}
  \text{Pure logic term} & \phi, \psi, \chi, \alpha & ::= &
  0 \mid \True \mid \mut \mid \imm \mid x \mid \phi = \phi \mid \phi \wedge \phi \mid \neg \phi 
  % \True \mid \False \mid e = e \mid
  % \\[2pt]
  % &&& \neg \phi \mid \phi \wedge \phi
  \\[2pt]
  \text{Symbolic heap} &\mcode{ P, Q, R} & ::= &
  \mcode{\emp \mid \ipointsto{e, \off}{e}{\iiann}
  \mid
  \iblock{e}{\off}{\iiann} \mid \mcode{\ipred{p}{\many{\phi_i}}{\many{\iiann_i}}}
      \mid P \sep Q}
  \\[2pt]
  \text{Heap predicate} & \indp & ::= &
  \mcode{\ipred{p}{\many{x_i}}{\many{\ann_j}}~\many{\pclause{\sel_k}{\chi_k}{R_k}}}
  \\[2pt]
  \text{Function spec} & \fun & ::= &
  \mcode{ f(\many{x_i}) : \asn{\slP} \asn{\slQ}}
  \\[2pt]
  % \text{Accessibility Annot.} & \mcode{\iiann} & ::= &
  % \mcode{\mut \mid \bimm{\ann} } % \mid \imm \mid A
  \text{Assertion} &  \slP, \slQ & ::= &
  \mcode{\set{\phi, P}}
  \\[2pt]
  \text{Environment} & \mcode{\env} & := &
  \mcode{  \epsilon \mid \env, x}
  \qquad ~
  \text{Context} \quad \mcode{\ctx} \quad  ~~~:= ~ \mcode{\epsilon \mid
    \ctx, \indp \mid \ctx, \fun}
  \\[2mm]
\end{array}
}
\]
%
\caption{\logicx assertion syntax.}
\label{fig:logic}
\end{figure}

\section*{Rules}

New rules of \logicx are shown in \autoref{fig:irules}.
%
Writing into a heap location requires this location to be explicitly annotated as mutable.
%
Note that if you have a precondition like 
${\asn{a = \mut ; \ipointsto{x}{5}{a}}}$,
we can first apply a normalization rule like \sleft to transform it into the form ${\asn{\mut = \mut ; \ipointsto{x}{5}{\mut}}}$,
at which point the \writer rule can be applied.
%
Note also that \allocr does not require specific permissions on the block in the postcondition;
if they turn out to be $\imm$, the resulting goal will be unsolvable,
but this way an existential permission would work.
%
\np{This is probably not how it's implemented, so feel free to change it
  back to $\mut$.} \ac{indeed it's not implemented this way. But I think
  it's ok to leave the formalism this way, since the implementation is just
  a prototype. We shall refine the implementation.}


\begin{figure}[!t]
\setlength{\belowcaptionskip}{-10pt}
\centering
{\footnotesize
\begin{mathpar}
\inferrule[\writer]
%
  % Γ ; {φ ; x.f -> l' * P} ; {ψ ; x.f -> l' * Q} ---> S   GV(l) = GV(l') = Ø
  % ------------------------------------------------------------------------- [write]
  % Γ ; {φ ; x.f -> l * P} ; {ψ ; x.f -> l' * Q} ---> *x.f := l' ; S
%
{
\mcode{\vars{e} \subseteq \env}
\qquad
\mcode{e \neq e'}
\\
\mcode{\env; \trans{{\asn{\phi ;
             \ipointsto{{x,\off}}{e}{\mut} \sep P}}}
{\asn{\psi;  \ipointsto{{x,\off}}{e}{\mut} \sep Q}} {\prog}
}}
{
  \mcode{\env;
    \trans
    {\asn{\phi; \ipointsto{{x,\off}}{e'}{\mut}  \sep P}}
    {\asn{\psi;  \ipointsto{{x,\off}}{e}{\mut} \sep Q}}
    {\deref{(x + \off)} = e; \prog}
  }
}
\\
\\
\inferrule[\allocr]
{
\mcode{  R = \iblock{z}{n}{{\iiann}} \sep \Sep_{0 \leq i < n}\paren{
    \ipointsto{z, i}{e_i}{\iiann_i}}
}
\qquad
\mcode{\paren{\set{y} \cup \set{\many{t_i}}} \cap \vars{\env, \slP, \slQ} = \emptyset}
\qquad
\mcode{z \in \ev{\env, \slP, \slQ}}
\\
\mcode{R' \eqdef \iblock{y}{n}{\mut} \sep \Sep_{0 \leq i < n}
  \paren{\ipointsto{y,i}{t_i}{\mut}}}
\\
\mcode{\ctx; \env; \trans{\asn{\phi; P \sep R'}}{\asn{\psi; Q \sep R}}{\prog}
}}
{
  \mcode{\ctx; \env;
  \trans
  {\asn{\phi; P}}
  {\asn{\psi; Q \sep \cached{R}}}
  {\Letz y = \malloc{n}; \prog}
}}
\\
\inferrule[\freer]
{
  \mcode{R = \iblock{x}{n}{{\mut}} \sep
    \Sep_{0 \leq i < n}\paren{
      \ipointsto{x,i}{e_i}{\mut} }}
 \qquad
 \mcode{\vars{\set{x} \cup \set{\many{e_i}}} \subseteq \env}
 \\
\mcode{\ctx; \env; \trans{\asn{\phi; P}}{\asn{\slQ}}{\prog}}
}
{\mcode{
\ctx; \env; \trans{\asn{\phi; P \sep \cached{R}}}{\asn{\slQ}}{\free{x}; \prog}
}}
\end{mathpar}
}
\caption{\logicx derivation rules.}
\label{fig:irules}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:



\section*{Memory Model}

The memory model follows closely the one introduced for Separation Logic
\cite{OHearn-al:CSL01,Reynolds:LICS02}.
We assume \mcode{\text{Loc} \subset \text{Val}}.
%
\begin{mathpar}
  \begin{array}{lrcl}
    \text{(Heap)}
    & \mcode{h \in \text{Heaps}}
    & \mcode{::=}
    & \mcode{\text{Loc} \rightharpoonup \text{{Val}}}
    \\
    \text{(Stack)}
    & \mcode{s \in \text{Stacks}}
    & \mcode{::=}
    & \mcode{\text{Var} \rightarrow \text{{Val}}}
  \end{array}
\end{mathpar}

To enable C-like accounting of dynamically-allocated memory blocks,
we will assume that the heap \mcode{h} can also store sizes of allocated blocks in dedicated locations
(conceptually, this part of the heap corresponds to the meta-data of the memory allocator).
This accounting is required to make sure that only a previously allocated memory block can be disposed (as opposed to any set of allocated locations),
and also enables the \mcode{free} command to accept a single argument: the address of the block.
To model this meta-data, we introduce a function \mcode{bl\colon \text{Loc}\to \text{Loc}},
where \mcode{bl(x)} denotes the location in the heap where the block meta-data for the address \mcode{x} is stored,
if \mcode{x} is the starting address of a block.
In an actual language implementation, \mcode{bl(x)} might be \eg\ \mcode{x - 1}
(\ie the meta-data is stored right before the block).

Since we have opted for an unsophisticated permission mechanism,
where the \emph{heap ownership is not divisible}, but some heap locations are restricted to
\mcode{\imm},
the definition of the satisfaction relation \mcode{\isatsl{}{}{\ilset}}
for the annotated assertions in a particular context \mcode{\ctx}
and given an interpretation \mcode{\interp}, is parameterized
with a fixed set of read-only locations, \mcode{\ilset}:
%
\begin{itemize}
\item \mcode{\isatsl{\angled{h, s}}{\asn{\phi; \emp}}{\ilset}}
  ~\Iff~
  \mcode{\denot{\phi}_s = \True} and \mcode{\dom{h} = \emptyset}.

\item \mcode{\isatsl{\angled{h, s}}{\asn{\phi;
        \ipointsto{e_1,\off}{e_2}{{\iiann}}}}{\ilset}}
  ~\Iff~
  %
  \mcode{\denot{\phi}_s = \True}
  %
  and \mcode{l\eqdef\denot{e_1}_s + \off}
  % 
  and \mcode{\dom{h} = \{l\}}
  %
  and \mcode{h(l) = \denot{e_2}_s}
  %
  % and (\mcode{\iiann=\mut \implies l\notin\ilset})
  and \textcolor{ACMRed}{\mcode{l\in\ilset \Leftrightarrow \iiann=\imm}}
  .
  
\item \mcode{\isatsl{\angled{h, s}}{\asn{\phi; \iblock{e}{\size}{\iiann}}}{\ilset}}
  ~\Iff~
  \mcode{\denot{\phi}_s = \True}
  %
  \textcolor{ACMRed}{
  and \mcode{l\eqdef bl(\denot{e}_s)}
  % 
  and \mcode{\dom{h} = \{l\}}
  %
  and \mcode{h(l) = \size}
  %
  and \mcode{l\in\ilset \Leftrightarrow \iiann=\imm}}.
  % 
  % and \mcode{
    % \forall i\in 0\ldots (n-1),
    % (\iiann=\mut \implies
    % (\denot{x}_s + i)
    % \notin\ilset)
    % }.
  

\item \mcode{\isatsl{\angled{h, s}}{\asn{\phi; P_1 \sep P_2 }}{\ilset}}  ~\Iff~
  \mcode{\exists~ h_1, h_2, h = h_1 \union h_2} and
  \mcode{\isatsl{\angled{h_1, s}}{\asn{\phi; P_1}}{\ilset}} and \\
  \mcode{\isatsl{\angled{h_2, s}}{\asn{\phi; P_2 }}{\ilset}}.

\item \mcode{\isatsl
    {\angled{h,s}}
    {\asn{\phi;\ipred{p}{\many{\psi_i}}{}}}
    {\ilset}}
  \Iff
  %
  \mcode{\denot{\phi}_s = \True}
  and \mcode{\indp \eqdef \ipred{p}{\many{x_i}}{}
    \many{\pclause{\sel_k}{\chi_k}{R_k}} \in \ctx}
  and\\
  \mcode{\angled{h,\many{\denot{\psi_i}_s}} \in \interp(\indp)}
  and \mcode{
  {\bigvee_{k}(
    \isatsl{\angled{h, s}}{[\many{\subs{x_i}{\psi_i}}]\asn{\phi \wedge \sel_k \wedge \chi_k; R_k}}{\ilset}
    )}}.
\end{itemize}

\textcolor{ACMRed}{
There are two non-standard cases: points-to and block, whose permissions must agree with \ilset.
Note that in the definition of satisfaction, we only need to consider that case where the permission $\iiann$ is a value (\ie either \mcode{\imm} or \mcode{\mut}).
Although in a specification $\iiann$ can also be a variable,
well-formedness guarantees that this variable must be logical, and hence will be substituted away in the definition of validity.
}

\np{I moved the invariant to the last theorem, since this is where we prove that it's preserved by any valid execution.
It is not true in general: \mcode{\slP} could be true in an empty heap, which certainly does not include all RO locations;
intuitively, \ilset\ is defined wrt the initial complete heap of the
program.}
\ac{yes, you're right, it is not true in general.}
% For a given model \mcode{\angled{h,s}} and assertion \mcode{\slP},
% the following invariant holds:\\
% \centerline{\mcode{inv(\isatsl{\angled{h, s}}{\asn{\slP}}{\ilset}) = \ilset
  % \subseteq \dom{h}}.}

We stress on the fact that a reference which has \mcode{\imm} permissions
to a certain symbolic heap, still retains the full ownership of that heap,
with the restriction that it is not allowed to update or deallocate it.
Note that deallocation additionally requires a mutable permission for the enclosing block.


\section*{Operational semantics}

The operational semantics is the traditional one \textcolor{ACMRed}{(but with blcok accounting in the rules \allocr and \freer)}:
\begin{center}
{
\footnotesize
\renewcommand{\arraystretch}{4}
$
\begin{array}{c}
  % \hspace{-5mm}
  \ebpsem{\writer}{{
      \Hypo{\mcode{
          (\denot{x}_s + \off) {\in} \dom{h}
          \qquad
          h'\eqdef h[(\denot{x}_s + \off) \rightarrow \denot{e}_s]
        }}
      \Infer1{\mcode{
          \opsem
          {\fctx}
          {\angled{h,(\deref{(x + \off)} = e ;\prog,s) \cdot S}}
          {\angled{h',(\prog,s) \cdot S}}
        }}
    }}
  \\
  \ebpsem{\readr}{{
      \Hypo{\mcode{
          (\denot{x}_s + \off) {\in} \dom{h}
          \qquad
          s'\eqdef s[y \rightarrow h(\denot{x}_s + \off)]
        }}
      \Infer1{\mcode{
          \opsem
          {\fctx}
          {\angled{h,(\Letz y = \deref{(x + \off);\prog},s) \cdot S}}
          {\angled{h,(\prog,s') \cdot S}}
        }}
    }}
  \\
  \ebpsem{\allocr}{{
      \Hypo{\mcode{
          y {\notin} \dom{s}
          \quad
          \exists l . bl(l) \notin \dom{h} \wedge
          \forall ~ i {\in} 0 {\ldots} \size - 1,
          ~
          (l{+}i) {\notin} \dom{h}         
        }}
      \Infer[no rule]1{\mcode{
          s' \eqdef s[y \rightarrow l]
          \quad
          h' \eqdef h\union (bl(l)\rightarrow \size) \union [(l{+}i) \rightarrow \_]
        }}
      \Infer1{\mcode{
          \opsem
          {\fctx}
          {\angled{h,(\Letz y = \malloc{\size};\prog,s) \cdot S}}
          {\angled{h',(\prog,s') \cdot S}}
        }}
    }}
  \\
  \ebpsem{\freer}{{
      \Hypo{\mcode{
          l \triangleq \denot{x}_s \quad
          \size \triangleq h(bl(l))
        }}
      \Infer[no rule]1{\mcode{
          h = h'\union (bl(l)\rightarrow \size) \union [(l{+}i) \rightarrow \_]
          % [\denot{x+0}_s \rightarrow \_
            % \ldots
            % \denot{x+(n-1)}_s \rightarrow \_]
        }}
      \Infer1{\mcode{
          \opsem
          {\fctx}
          {\angled{h,(\free{x};\prog,s) \cdot S}}
          {\angled{h',(\prog,s) \cdot S}}
        }}
    }}
  \\
  \ebpsem{\applyr}{{
      \Hypo{\mcode{
          f(\many{x_i})\{\prog'\} \in \fctx
          \quad
          s' \eqdef [x_i \rightarrow \denot{y_i}_s]
        }}
      \Infer1{\mcode{
          \opsem
          {\fctx}
          {\angled{h,(f(\many{y_i});\prog,s) \cdot S}}
          {\angled{h', (\prog',s') \cdot (\prog,s) \cdot S}}
        }}
    }}
\end{array}
$
}
\end{center}

\section*{Soundness}

The validity definition and the soundness proofs of \logic are ported to
\logicx without any modification, since our current definition of
satisfaction implies the one defined for \logic.
%
\np{Not quite true anymore because of blocks in OS and satisfaction,
but they should be trivial and also irrelevant to the substance of this paper, so I suggest we gloss over that.}

\begin{definition}[Validity]
  \label{def:validity}
  We say that a well-formed Hoare-style specification
  \mcode{\ctx; \env; \asn{\slP}~\prog~\asn{\slQ}} is \emph{valid} \wrt the
  function dictionary \mcode{\fctx} \Iff
  %
  whenever
  %
  \mcode{\dom{s} = \env},
  %
  \mcode{\forall \subst_{\text{gv}} = [\many{x_i \mapsto d_i}]_{x_i \in \gv{\env, \slP,
      \slQ}}}
  such that
  \mcode{\satsl{\angled{h, s}}{[\subst_{\text{gv}}]\slP}},  and
  %
  %
  \mcode{\opsemt{\fctx}{\angled{h, (c, s) \cdot \epsilon}}{\angled{h',
      (\ccd{skip}, s') \cdot \epsilon}}},
  %
  it is also the case that
  %
  \mcode{\satsl{\angled{h', s'}}{[\subst_{\text{ev}} \union
      \subst_{\text{gv}}]}\slQ}
  %
  for some \mcode{\subst_{\text{ev}} = [\many{y_j \mapsto d_j}]_{y_j \in \ev{\env,
      \slP, \slQ}}}.
\end{definition}

\np{I'm a bit confused by the $\exists \subst_{\text{gv}}$ in this definition:
maybe I got mixed up with logical connectives, but don't we want the program to run correctly for \emph{any} assignment to ghost vars
that satisfies the starting heap, not just some assignment?} \ac{agree, i
changed to \mcode{\forall}}.

\begin{theorem}[RO Heaps Do Not Change]
\label{thm:ro-heaps}
Given a Hoare-style specification
%
\mcode{\ctx; \env;
  {\asn{\phi;P}}
  {\prog}
  {\asn{\slQ}}
},
%
which is valid \wrt the function dictionary
% 
\mcode{\fctx},
%
and a set of read-only memory locations \mcode{\ilset},
if:
  %
  \begin{enumerate}[label=\emph{(\roman*)}]
    % 
  \item
    \mcode{\isatsl{\angled{h, s}}{[\subst]\slP}{\ilset}},
    for some 
    \mcode{\mcode{h,s}}
    and
    \mcode{\subst},
    and
    % 
  \item
    \mcode{\opsemt{\fctx}
      {\angled{h, (c, s) \cdot \epsilon}}
      {\angled{h',(c', s') \cdot \epsilon}}}
    %
    for some 
    \mcode{h',s'}
    and
    \mcode{c'}
  \item
    \mcode{\ilset \subseteq \dom{h}}
  \end{enumerate}
  %
  then 
  \mcode{\ilset \subseteq \dom{h'}}
  and
  \mcode{\forall l \in \ilset,~ h(l) = h'(l).}
\end{theorem}
\begin{proof}
  Our proof strategy is to prove that if
  \mcode{\isatsl{}{}{\ilset}} holds and
  \mcode{\Opsem} modifies some memory locations, then those
  locations are not in \mcode{\ilset}.
  %
  The theorem then follows by induction on \mcode{\Opsemt}.
  %
  For brevity, we only show the base cases for the heap update:\\
  %
  \noindent{\bf Case:} \mcode{\writer}. Assume that
  (1) \mcode{\isatsl{\angled{h, s}}
    {[\subst]\ipointsto{x + \off}{\_}{\iiann} \sep P'}{\ilset}},
  %
  and also that 
  (2) \mcode{\opsemt{\fctx} 
    {\angled{h, (\deref{(x + \off)} = e;\prog, s) \cdot \epsilon}}
    {\angled{h',(\prog, s') \cdot \epsilon}}}.
  %
  Assuming in (1) that \mcode{\iiann \neq \mut},
  % 
  contradicts the validity assumption of
  \mcode{\ctx; \env;
    {\asn{\phi;P}}
    {\deref{(x + \off)} = e;\prog}
    {\asn{\slQ}}
  }, therefore \mcode{\iiann=\mut}.
  %
  By (i) and \mcode{\iiann=\mut}, it follows that 
  (3) \mcode{(\denot{x}_s + \off) \notin \ilset}.
  %
  By (1) it follows that 
  (4) \mcode{h'=h[(\denot{x}_s + \off) \rightarrow \denot{e}_s]}.
  % 
  Finally, by (3) and (4) it follows that
  \mcode{\forall l \in \ilset,~ h(l) = h'(l).}
  %
  In addition, since \mcode{dom(h) = dom(h')}, then from (iii) it follows that \mcode{\ilset \subseteq \dom{h'}}.\\
  %
  \noindent{\bf Case:} \mcode{\allocr}. Assuming that
  \mcode{\opsemt{\fctx} 
    {\angled{h, (\Letz y = \malloc{\size};\prog, s) \cdot \epsilon}}
    {\angled{h',(\prog, s') \cdot \epsilon}}},
  it follows then that 
  %
  (1)
  {\mcode{
      \forall ~ i {\in} 0 {\ldots} \size{-}1,
      ~
      (l{+}i) {\notin} \dom{h}
      ~\text{and}~
      bl(l) \notin \dom(h)
      ~\text{and}~
      h' \eqdef h\union(bl(l) \rightarrow \size)\union[(l{+}i) \rightarrow \_]
    }}.
  %
  From (1) and (iii) we conclude that
  that \mcode{\forall l \in \ilset,~ h(l) = h'(l).}
  %
  In addition, since \mcode{dom(h) \subset dom(h')}, then from (iii) it follows that \mcode{\ilset \subseteq \dom{h'}}.\\
  %
  \noindent{\bf Case:} \mcode{\freer}. 
  Assuming that
  \mcode{
          \opsem
          {\fctx}
          {\angled{h,(\free{x};\prog,s) \cdot S}}
          {\angled{h',(\prog,s) \cdot S}}
        }
  we get (1) \mcode{h = h'\union (bl(l)\rightarrow \size) \union [(l{+}0) \rightarrow \_ \ldots (l{+}\size - 1) \rightarrow \_]} 
  (where \mcode{l \triangleq \denot{x}_s} and \mcode{\size \triangleq h(bl(l))}):
  hence the values stored in the heap are not modified, and it is only left to prove that \mcode{\ilset \subseteq \dom{h'}},
  \ie that \mcode{bl(l) \notin \ilset} and \mcode{(l{+}i) \notin \ilset} for \mcode{i \in 0\ldots \size - 1}.
  %
  By validity and (i), we have (2) 
  \mcode{\isatsl{\angled{h, s}}{[\subst](\iblock{x}{n}{{\mut}} \sep
    \Sep_{0 \leq i < n}\paren{
      \ipointsto{x,i}{e_i}{\mut} } ) \sep P'}{\ilset}}.
  The rest follows from (2) and the definition of satisfaction.
  % Assume that
  % %
  % \mcode{\isatsl{\angled{h, s}}{\asn{\phi; \iblock{x}{n}{\iiann} \sep
        % P'}}{\ilset}}.
  % %
  % Taking \mcode{\iiann\neq\mut} contradicts the validity of the triple,
  % hence \mcode{\iiann=\mut}.
  % %
  % By (i) and \mcode{\iiann=\mut}, it follows that 
  % (1) \mcode{\forall i \in 0\ldots(n-1), (\denot{x}_s + i) \notin \ilset}.
  % %
  % Assuming that
  % \mcode{\opsemt{\fctx} 
    % {\angled{h, (\free{x};\prog, s) \cdot \epsilon}}
    % {\angled{h',(\prog, s) \cdot \epsilon}}},
  % %
  % it follows that
  % (2) \mcode{
    % h = h'\union[\denot{x+0}_s \rightarrow \_
      % \ldots
      % \denot{x+(n-1)}_s \rightarrow \_].
  % }
  % % 
  % From (1) and (2) we conclude that
  % that \mcode{\forall l \in \ilset,~ h(l) = h'(l).}
  \qed
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper-formal-2"
%%% End:


==> auxiliary_proofs.tex <==


~\\
\noindent\emph{\bf Memory model with Accessibility Permissions.}
The memory model follows closely the one introduced for Separation Logic
\cite{OHearn-al:CSL01,Reynolds:LICS02}, with the adjustments on
heaps which are partial functions from sets of locations to pairs of values
and accessibility annotations:
\begin{mathpar}
  \begin{array}{llcl}
    \text{(Accessibility Annotation)\quad}
    & \mcode{\iiann \in \text{Imm}}
    & \mcode{::=}
    & \mcode{ \{\mut,\bimm{\ann}\} }\\
    \text{(Heap)}
    & \mcode{h \in \text{Heaps}}
    & \mcode{::=}
    & \mcode{\text{Loc} \rightarrow \text{ObjVal} \times \text{Imm}}\\
    \text{(Stack)}
    & \mcode{s \in \text{Stacks}}
    & \mcode{::=}
    & \mcode{\text{Var} \rightarrow \text{Val} \cup \text{Loc}}
  \end{array}
\end{mathpar}

Since we have opted for an unsophisticated permission mechanism,
where the \emph{heap ownership is not divisible}, but just restricted to
\mcode{\imm} at times,
the definition
of the satisfaction relation \mcode{\satsl{}{}}
for the annotated assertions in a particular context \mcode{\ctx}
and given an interpretation \mcode{\interp} is straightforward:
\begin{itemize}
\item \mcode{\satsl{\angled{h, s}}{\asn{\phi; \emp}}}
  ~\Iff~
  \mcode{\denot{\phi}_s = \True} and \mcode{\dom{h} = \emptyset}.

\item \mcode{\satsl{\angled{h, s}}{\asn{\phi; \iblock{x}{n}{\iiann}}}}
  ~\Iff~
  \mcode{\denot{\phi}_s = \True} and \mcode{\dom{h} = \emptyset}.

\item \mcode{\satsl{\angled{h, s}}{\asn{\phi;
        \ipointsto{e_1,\off}{e_2}{{\iiann}}}}}
  ~\Iff~
  \mcode{\denot{\phi}_s = \True} and \mcode{\dom{h} = \denot{e_1}_s + \off}
  and \\
  \mcode{h(\denot{e_1}_s + \off) = (\denot{e_2}_s,\iiann')}
  and
  (\mcode{\iiann' = M ~\text{or}~ \iiann' = \iiann})
  .

\item \mcode{\satsl{\angled{h, s}}{\asn{\phi; P_1 \sep P_2 }}}  ~\Iff~
  \mcode{\exists~ h_1, h_2, h = h_1 \union h_2} and
  \mcode{\satsl{\angled{h_1, s}}{\asn{\phi; P_1}}} and \\
  \mcode{\satsl{\angled{h_2, s}}{\asn{\phi; P_2 }}}.

\item \mcode{\satsl{\angled{h, s}}{\asn{\phi; p(\many{x_i},{\many{\iiann_j}})}}} \Iff
  \mcode{\denot{\phi}_s = \True} and
  \mcode{\indp \eqdef p(\many{x'_i},{{\many{\ann'_j}}}) \many{\pclause{\sel_k}{\chi_k}{R_k}} \in \ctx} and
  \mcode{\angled{h, \many{\denot{x_i}_s}} \in \interp(\indp)}
  and \mcode{
  {\bigvee_{k}(
    \satsl{\angled{h, s}}{[\many{\subs{x'_i}{x_i}}],[\many{\subs{\ann'_j}{\iiann_j}]}\asn{\phi \wedge \sel_k \wedge \chi_k; R_k)}}
    )}}.
\end{itemize}

We next define the following equality predicate (equality on the values,
but not on the permissions) for heaps:
\[
\begin{array}{lcl}
  \mcode{h_1 =_{\%} h_2 } &\text{iff}&
  \mcode{\dom{h_1} = \dom{h_2} = D}
  ~\text{and}~\\
  &&
  \mcode{\forall l \in D, h_1(l)=(v,\_) }
  ~\text{and}~
  \mcode{h_2(l)=(v,\_) }.
\end{array}
\]
We next define a merge operator which takes the values from the first heap,
and the permission from the second heap, to merge them into one new heap:
\[
\begin{array}{lcl}
  \mcode{h_1 \oplus h_2 } &\defeq&
  \mcode{[l \rightarrow (v,\iiann) | l \in D ~\text{and}~ h_1(l)=(v,\_)
    ~\text{and}~ h_2(l)=(\_,\iiann)
    ].}
\end{array}
\]

\noindent defined only when \mcode{\dom{h_1} \subseteq \dom{h_2}}.

We stress on the fact that a reference which has \mcode{\imm} permissions
to a certain symbolic heap, still retains the full ownership of that heap,
with the restriction that it is not allowed to update or deallocate it.
Bearing this in mind, below are some selected instrumented
\footnote{the semantic is instrumented to explicitly track for the
  accessibility permission.}
operational semantics rules:

{
\footnotesize
\renewcommand{\arraystretch}{4}
$
\begin{array}{c}
  % \hspace{-5mm}
  \ebpsem{\writer}{{
      \Hypo{\mcode{
          (\denot{x}_s + \off) {\in} \dom{h}
          \qquad
          h(\denot{x}_s + \off) = (\_,\mut)
          \qquad
          h'\eqdef h[(\denot{x}_s + \off) \rightarrow (\denot{e}_s,\mut)]
        }}
      \Infer1{\mcode{
          \opsem
          {\fctx,\ctx}
          {\angled{h,(\deref{(x + \off)} = e,s) \cdot S}}
          {\angled{h',(\cskip,s) \cdot S}}
        }}
    }}
  \\
  \ebpsem{\readr}{{
      \Hypo{\mcode{
          (\denot{x}_s + \off) {\in} \dom{h}
          \qquad
          h(\denot{x}_s + \off) = (v,\_)
          \qquad
          s'\eqdef s[y \rightarrow v]
        }}
      \Infer1{\mcode{
          \opsem
          {\fctx;\ctx}
          {\angled{h,(\Letz y = \deref{(x + \off)},s) \cdot S}}
          {\angled{h,(\cskip,s') \cdot S}}
        }}
    }}
  \\
  \ebpsem{\allocr}{{
      \Hypo{\mcode{
          y {\notin} \dom{s}
          \quad
          \exists l {\notin} \dom{h}
          \quad
          s' \eqdef s[y \rightarrow l]
        }}
      \Infer[no rule]1{\mcode{
          \forall ~ i {\in} 0 {\ldots} \denot{n{-}1}_s,
          ~
          (l{+}i) {\notin} \dom{h}
          \quad
          h' \eqdef h\union[(l{+}i) \rightarrow (\_,\mut)]
        }}
      \Infer1{\mcode{
          \opsem
          {\fctx;\ctx}
          {\angled{h,(\Letz y = \malloc{n},s) \cdot S}}
          {\angled{h',(\cskip,s') \cdot S}}
        }}
    }}
  \\
  \ebpsem{\freer}{{
      \Hypo{\mcode{
          \exists x {\in} \dom{s}
          \quad
          \exists n ~~
          \satsl{\angled{h, s}}{\iblock{x}{n}{\mut}}
        }}
      \Infer[no rule]1{\mcode{
          h = h'\union[\denot{x+0}_s \rightarrow (\_,M)
            \ldots
            \denot{x+(n-1)}_s \rightarrow (\_,M)]
        }}
      \Infer1{\mcode{
          \opsem
          {\fctx;\ctx}
          {\angled{h,(\free{x},s) \cdot S}}
          {\angled{h',(\cskip,s) \cdot S}}
        }}
    }}
  \\
  \ebpsem{\applyr}{{
      \Hypo{\mcode{
          f(\many{x_i})\{c\} \in \fctx
          \quad
          s' \eqdef [x_i \rightarrow \denot{y_i}_s]
          \quad
          f(\many{x_i}){\asn{\slP}}{\asn{\slQ}} \in \ctx
          \quad
          h = h_1 \union h_2
        }}
      \Infer[no rule]1{\mcode{
          \opsem
          {\fctx;\ctx}
          {\angled{\emptyset,(assert(\slP),s') \cdot \epsilon}}
          {\angled{h'_2,(\cskip,s') \cdot \epsilon}}
          \qquad
          h''_2 \eqdef h_2 \oplus h'_2 
        }}
      \Infer[no rule]1{\mcode{
          \opsem
          {\fctx;\ctx}
          {\angled{h''_2,(c,s') \cdot \epsilon}}
          {\angled{h'''_2,(\cskip,s') \cdot \epsilon}}
          \qquad
          h' \eqdef h_1 \union (h'''_2 \oplus h_2)
        }}
      \Infer1{\mcode{
          \opsem
          {\fctx;\ctx}
          {\angled{h,(f(\many{y_i}),s) \cdot S}}
          {\angled{h',(\cskip,s) \cdot S}}
        }}
    }}
\end{array}
$
}

Clearly, this is not a realistic machine,
since it rejects programs based
on the accessibility information, on top of requiring extra instructions
(\code{assume})
to account for the accessibility annotations once
a call is initiated.
% , while a real machine would not have this
% information available.
But this is not an issue, since we can define an
erasure function \cite{hobor2011barriers} to map instrumented states
to sets of concrete states. The real machine
\cite{Polikarpova-Sergey:POPL19} takes no decision
based on read-only information, hence the instrumented semantics simply rejects
more executions than the real machine. This is also the informal argument
for which the termination results of \logic
directly apply to \logicx, since the latter
conservatively narrows the space of accepted derivations.


The soundness proof of \logic carries over to accessibility annotated-heaps
with no difficulty, since it is reduced to showing that
whenever the instrumented semantics takes a step
\mcode{ \opsem {\fctx;\ctx}
{\angled{h, (c,s), \cdot S}}
{\angled{h',(\cskip,s') \cdot S}}
}
then the erased semantics, correspondingly, steps
\mcode{
  \opsem
  {\fctx}
  {\angled{erase(h), (c,s), \cdot S}}
  {\angled{erase(h'),(\cskip,s') \cdot S}}
},
where \mcode{erased(h) \defeq {[l\rightarrow v|
      l\in \dom{h} ~\text{and}~ h(h)=(v,\_)]}}.

The erased semantics is the traditional one:

{
\footnotesize
\renewcommand{\arraystretch}{4}
$
\begin{array}{c}
  % \hspace{-5mm}
  \ebpsem{\writer}{{
      \Hypo{\mcode{
          (\denot{x}_s + \off) {\in} \dom{h}
          \qquad
          h'\eqdef h[(\denot{x}_s + \off) \rightarrow \denot{e}_s]
        }}
      \Infer1{\mcode{
          \opsem
          {\fctx}
          {\angled{h,(\deref{(x + \off)} = e,s) \cdot S}}
          {\angled{h',(\cskip,s) \cdot S}}
        }}
    }}
  \\
  \ebpsem{\readr}{{
      \Hypo{\mcode{
          (\denot{x}_s + \off) {\in} \dom{h}
          \qquad
          s'\eqdef s[y \rightarrow h(\denot{x}_s + \off)]
        }}
      \Infer1{\mcode{
          \opsem
          {\fctx}
          {\angled{h,(\Letz y = \deref{(x + \off)},s) \cdot S}}
          {\angled{h,(\cskip,s') \cdot S}}
        }}
    }}
  \\
  \ebpsem{\allocr}{{
      \Hypo{\mcode{
          y {\notin} \dom{s}
          \quad
          \exists l {\notin} \dom{h}
          \quad
          s' \eqdef s[y \rightarrow l]
        }}
      \Infer[no rule]1{\mcode{
          \forall ~ i {\in} 0 {\ldots} \denot{n{-}1}_s,
          ~
          (l{+}i) {\notin} \dom{h}
          \quad
          h' \eqdef h\union[(l{+}i) \rightarrow \_]
        }}
      \Infer1{\mcode{
          \opsem
          {\fctx}
          {\angled{h,(\Letz y = \malloc{n},s) \cdot S}}
          {\angled{h',(\cskip,s') \cdot S}}
        }}
    }}
  \\
  \ebpsem{\freer}{{
      \Hypo{\mcode{
          \exists x {\in} \dom{s}
          \quad
          \exists n ~~
          \satsl{\angled{h, s}}{\iblock{x}{n}{}}
        }}
      \Infer[no rule]1{\mcode{
          h = h'\union[\denot{x+0}_s \rightarrow \_
            \ldots
            \denot{x+(n-1)}_s \rightarrow \_]
        }}
      \Infer1{\mcode{
          \opsem
          {\fctx}
          {\angled{h,(\free{x},s) \cdot S}}
          {\angled{h',(\cskip,s) \cdot S}}
        }}
    }}
  \\
  \ebpsem{\applyr}{{
      \Hypo{\mcode{
          f(\many{x_i})\{c\} \in \fctx
          \quad
          s' \eqdef [x_i \rightarrow \denot{y_i}_s]
        }}
      \Infer1{\mcode{
          \opsem
          {\fctx}
          {\angled{h,(f(\many{y_i}),s) \cdot S}}
          {\angled{h', (c,s') \cdot (\cskip,s) \cdot S}}
        }}
    }}
\end{array}
$
}


\begin{definition}[Well-Formedness of Spatial Predicates]
  \label{def:well-formed-pred}
  We say that a spatial predicate
  \mcode{\ipred{p}{\many{x_i}}{\many{\ann_j}}~\many{\pclause{\sel_k}{\chi_k}{R_k}}_{k\in 1..N}}
  is \emph{well-formed} \Iff
  \begin{enumerate}[label=\emph{(\roman*)}]
  \item \mcode{(\bigcup_{k=1}^{N} (\vars{\sel_k} \cup \vars{\chi_k} \cup \vars{R_k} ) \cap \iset)
  \subseteq
  (\many{x_i} \cap \iset)} %, and
  % \item \mcode{\forall k \in 1..N,
	% R_k = \ipred{p}{\many{y_i}}{\many{\ann'_j}} \sep R_k'
  %   \implies
  %   (\bigwedge_i {x_i \in \iset \implies (x_i = y_i)})}.
 \end{enumerate}
\end{definition}

That is, every accessibility annotation within the predicate's clause is
bound by one of the predicate's  parameters, and every inductive
instance of the predicate bears the same accessibility pattern with
the predicate header.

\begin{definition}[Well-Formedness of Specifications]
  \label{def:well-formed-spec}
  We say that a Hoare-style specification
  $\ctx; \env; \asn{\slP}~c~\asn{\slQ}$ is \emph{well-formed} \Iff
  \mcode{~\ev{\env,\slP, \slQ} \cap \iset = \emptyset}
  and every predicate instance
  in \mcode{\slP} and \mcode{\slQ} is an instance of a
  well-formed predicate.
\end{definition}

That is, postconditions are not allowed to have existential accessibility
annotations in order to avoid permanent weakening/strengthening of
accessibility.

\begin{definition}[Validity]
  \label{def:validity}
  We say that a well-formed Hoare-style specification
  $\ctx; \env; \asn{\slP}~c~\asn{\slQ}$ is \emph{valid} \wrt the
  function dictionary $\fctx$ \Iff
  %
  whenever
  %
  $\dom{s} = \env$,
  %
  $\exists \subst_{\text{gv}} = [\many{x_i \mapsto d_i}]_{x_i \in \gv{\env, \slP,
      \slQ}}$
  such that
  $\satsl{\angled{h, s}}{[\subst_{\text{gv}}]\slP}$,  and
  %
  %
  $\opsemt{\fctx}{\angled{h, (c, s) \cdot \epsilon}}{\angled{h',
      (\ccd{skip}, s') \cdot \epsilon}}$,
  %
  it is also the case that
  %
  $\satsl{\angled{h', s'}}{[\subst_{\text{ev}} \union
      \subst_{\text{gv}}]}\slQ$
  %
  for some $\subst_{\text{ev}} = [\many{y_j \mapsto d_j}]_{y_j \in \ev{\env,
      \slP, \slQ}}$.
\end{definition}

The notion of Hoare-style validity given in  \autoref{def:validity}
is easily ported from \logic to \logicx in  the
presence of well-formedness specifications, since
\mcode{dom(\subst_{\text{ev}}) \cap \iset = \emptyset}.

% \logicx actually benefits from all of \logic formal guarantees
% 1. show that when starting with \mcode{\imm} as a state then  \mcode{\imm} is
% either preserved for that heap, or the synthesis fails.

We next need to show that any command which requires immutable
accessibility, after being executed, it returns the borrow. This is trivial
for all cases except for \mcode{\applyr} rules, since no other rule
may require a weakening of the accessibility.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper-formal"
%%% End:


==> case.tex <==

\section{Case Study}
\label{sec:case}

It would be nice to have a new case study here, \eg, a skip-list. Can we copy it or flatten into an ordinary list?



==> fig/eq.tex <==
\begin{figure}[t]
\centering
{\footnotesize
 \begin{mathpar}
   \inferrule[]
   {
     \mcode{\block{x}{n_1} {=_s} [\subst]
            \block{y}{n_2}
     }
     \qquad
     \mcode{{{\iiann}_1} {=} {{{\iiann}_2}}}
   }{
     \mcode{%\eset ;
       \iblock{x}{n_1}{\iiann_1}
       \seq
       [\subst]\!\iblock{y}{n_2}{{{\iiann}_2}}
       }
   }
   \qquad
   \inferrule[]
   {
     \mcode{\pointsto{x,\off_1}{e_1} {=_s}
       [\subst']\!
       \pointsto{y,\off_2}{e_2}
     }
     \qquad
     \mcode{{{\iiann}_1} {=} {{{\iiann}_2}} }
   }{
     \mcode{%\eset ;
       \ipointsto{x,\off_1}{e_1}{\iiann_1}
       \seq
       [\subst]\!\ipointsto{y,\off_2}{e_2}{{{\iiann}_2}}
     }
   }\\
   \inferrule[]
   {
     \mcode{
       \spred{p}{\many{x_i}}
       {=_s} [\subst]
       \spred{p}{\many{y_i}}
       }
     \qquad
     \mcode{\forall
       \iiann_i' {\in} \many{\iiann}_i' ,
       \iiann_i {\in} \many{\iiann}_i
       \cdot
       {\iiann_i} {=} {\iiann_i'}}
   }{
     \mcode{\ipred{p}{\many{x_i}}{\many{\iiann_i}}
       {\seq} [\subst]
       \ipred{p}{\many{y_i}}{\many{\iiann_i'}}
     }
   }
\end{mathpar}
}
\caption{Selected rules for equality check in the presence of immutability.} \label{fig:seq}
\end{figure}


\begin{figure}[t]
\centering
{\footnotesize
 \begin{mathpar}
   \inferrule[\borrowr-Block]
   {
     \mcode{\block{x}{n_1} {=_s} [\subst']
            \block{y}{n_2}
     }
     \qquad
     \mcode{\subst {=} [\subst',\subs{{\bimm{\ann}}}{{\iiann}}]}
   }{
     \mcode{%\eset ;
       \iblock{x}{n_1}{\iiann}
       \ieq
       [\subst]\!\iblock{y}{n_2}{{\bimm{\ann}}}
       }
   }
   \qquad
   \inferrule[]
   {
     \mcode{\block{x}{n_1} {=_s} [\subst]
       \block{y}{n_2}
     }
     \qquad
     \mcode{\subann{\iiann}{\mut}}
   }{
     \mcode{%\eset ;
       \iblock{x}{n_1}{\iiann}
       \ieq
       [\subst]\!\iblock{y}{n_2}{\mut}
     }
   }
   \\
   \inferrule[\borrowr-PtsTo]
   {
     \mcode{\pointsto{x,\off_1}{e_1} {=_s}
       [\subst']\!
       \pointsto{y,\off_2}{e_2}
     }
     \qquad
     \mcode{\subst {=} [\subst',\subs{{\bimm{\ann}}}{{\iiann}}]}
   }{
     \mcode{%\eset ;
       \ipointsto{x,\off_1}{e_1}{\iiann}
       \ieq
       [\subst]\!\ipointsto{y,\off_2}{e_2}{{\bimm{\ann}}}
     }
   }
   \qquad
   \inferrule[]
   {
     \mcode{\pointsto{x,\off_1}{e_1} {=_s}
       [\subst]\!
       \pointsto{y,\off_2}{e_2}
     }
     \qquad
     \mcode{\subann{\iiann}{\mut}}
   }{
     \mcode{%\eset ;
       \ipointsto{x,\off_1}{e_1}{\iiann}
       \ieq
       [\subst]\!\ipointsto{y,\off_2}{e_2}{\mut}
     }
   }
   \\
   \inferrule[\borrowr-Pred]
   {
     \mcode{
       \spred{p}{\many{x_i}}
       {=_s} [\subst']
       \spred{p}{\many{y_i}}
       }
     \qquad
     \mcode{\subst = [\subst'] \cup
       [\subs{\bimm{\ann}'_i}{\iiann_i} ~|~ \iiann_i {\in} \many{\iiann_i}
         \text{~and~}  \bimm{\ann}_i' {\in} \many{\bimm{\iiann}_i'} ]}
     \\
     \mcode{\forall
       {\iiann}_i' {\in} \many{\bimm{\iiann}}_i' ,
       \iiann_i {\in} \many{\iiann}_i
       \cdot
       \subann{{\iiann}_i'}{\mut}
       \Rightarrow \subann{\iiann_i}{\mut} }
   }{
     \mcode{\ipred{p}{\many{x_i}}{\many{\iiann_i}}
       {\ieq} [\subst]
       \ipred{p}{\many{y_i}}{\many{\iiann_i'}}
     }
   }
\end{mathpar}
}
\caption{Selected rules for subsumption check in the presence of immutability.} \label{fig:ieq}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:


==> fig/simple-eq.tex <==
\begin{figure}[t]
\setlength{\belowcaptionskip}{-10pt}
\centering
{\footnotesize
 \begin{mathpar}
   \inferrule[]
   {
     \mcode{P  {=_s} [\subst]Q}
     \qquad
     \mcode{{\ann_P}{=}{\ann_Q}}
     \qquad
     \mcode{\ann_Q \notin \eset}
   }{
     \mcode{\eset ;~ P\iann{\ann_P} \seq
       [\subst]Q\iann{\ann_Q}}
   }
   \qquad
   \inferrule[]
   {
     \mcode{P  {=_s} [\subst']Q}
     \qquad
     \mcode{\ann_Q \in \eset}
     \qquad
     \mcode{\subst \eqdef [\subst',\subs{\ann_Q}{\ann_P}]}
   }{
     \mcode{\eset ;~ P\iann{\ann_P} \seq
       [\subst]Q\iann{\ann_Q}}
   }
\end{mathpar}
}
\caption{Selected rules for equality check in the presence of immutability
  (the left-hand side is used for framing, and the right-hand side for abduce).} \label{fig:simple-seq}
\end{figure}

\begin{figure}[t]
\centering
{\footnotesize
 \begin{mathpar}
   \inferrule[\borrowr]
   {
     \mcode{P  {=_s} [\subst']Q}
     \qquad
     % \mcode{\subann{\ann_P}{\imm}}
     % \qquad
     \mcode{\subst = [\subst',\subs{\bimm{\ann}_Q}{\ann_P}]}
%     \qquad
%     \mcode{\ann_Q \in \eset}
   }{
     \mcode{%\eset ;
       ~ P\iann{\ann_P} \ieq
       [\subst]Q\iann{\bimm{\ann}_Q}}
   }
   \qquad
   \inferrule[]
   {
     \mcode{P  {=_s} [\subst]Q}
     \qquad
     \mcode{\subann{\ann_P}{\mut}}
   }{
     \mcode{%\eset ;~
       P\iann{\ann_P} \ieq
       [\subst]Q\iann{\mut}}
   }
   % \qquad
   % \inferrule[]
   % {
   %   \mcode{P  {=_s} [\subst]Q}
   %   \qquad
   %   \mcode{\subann{\ann_P}{\imm}}
   % }{
   %   \mcode{\eset ;~ P\iann{\ann_P} \ieq
   %     [\subst]Q\iann{\imm}}
   % }
   % % \qquad
   % \inferrule[]
   % {
   %   \mcode{P  {=_s} [\subst']Q}
   %   \qquad
   %   \mcode{\ann_Q \in \eset}
   %   \qquad
   %   \mcode{\subst \eqdef [\subst',\subs{\ann_Q}{\ann_P}]}
   % }{
   %   \mcode{\eset ;~ P\iann{\ann_P} \ieq
   %     [\subst]Q\iann{\ann_Q}}
   % }
\end{mathpar}
}
\caption{Selected rules for subsumption check in the presence of immutability.} \label{fig:simple-ieq}
\end{figure}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:


==> optimizations.tex <==
\section{Optimisations}
\label{sec:optimisations}

\subsection{Favour Immutable Heap Unifications}
When the synthesis discovers multiple candidates for heap unifications,
it prioritizes those that are immutable since their data should be
compatible for unification.
To highlihgt the benefit of doing this let us revisit  the goal in
\ref{subsec:reduce-nondet}. Should the synthesizer
first choose to unify the heaplet pointed by \mcode{x},
it would result in the following derivation:
\begin{center}
  {\centering
  \footnotesize{
\begin{prooftree}
\Hypo[]
{
  \begin{array}{c}
    \mcode{\neg{(\subann{\bimm{\ann}}{\mut})}}
  \end{array}
}
\Infer1[\writer]
{
  \begin{array}{c}
    \mcode{\set{x, y};
      \trans
      {\asn{ \ispointsto{y}{30}{\bimm{\ann}}}}
      {\asn{ \ispointsto{y}{239}{\bimm{\ann}} }}
      {\prog_3}}
    \\[3pt]
    \mcode{\prog_2 = \prog_3}
  \end{array}
}
\Infer1[\framer]
{
  \begin{array}{c}
    \mcode{\set{x, y};
      \trans
      {\asn{ \gbm{\ispointsto{x}{239}{\mut}} \sep \ispointsto{y}{30}{\bimm{\ann}}}}
      {\asn{ \gbm{\ispointsto{x}{239}{\mut}} \sep \ispointsto{y}{239}{\bimm{\ann}} }}
      {\prog_2}}
    \\[3pt]
    \mcode{[\subs{z}{239}]\ispointsto{x}{z}{\mut} = \ispointsto{x}{239}{\mut}}
    \qquad
    \mcode{\prog_1 = \prog_2}
  \end{array}
}
\Infer1[\hunir]
{
  \mcode{
    \set{x, y};
    \trans
    {\asn{ \gbm{\ispointsto{x}{239}{\mut}} \sep \ispointsto{y}{30}{\bimm{\ann}}}}
    {\asn{ \gbm{\ispointsto{x}{z}{\mut}} \sep \ispointsto{y}{z}{\bimm{\ann}} }}
    {\prog_1}
  }
}
\end{prooftree}
}}
\end{center} 

The above process is stuck when 
attempting to write at the location pointed
by \mcode{y}  since \mcode{y} does not have the necessary permissions to do
so. The synthesizer thus backtracks and attempts a different heap
unification, namely that which involves the \mcode{y} reference,
which now succeeds (see the appendix for the full derivation). 
The first attempt on the unification of the heap pointed by \mcode{x}
is a nuisance in this case.
It is thus sensible to favor the unification of immutable
heaplets over the mutable one since this strategy reduces
the number of backtrackings in the presence of immutability annotations.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> tables/tab2-robustness.tex <==
\begin{table}[t]
\begin{center}
\tiny

\input{tables/table2}

\end{center}
\caption{\todo{ change the file name to description}}
\label{fig:evaluation}
\end{table}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:


==> tables/table2.tex <==
\begin{tabular}{@{} c | c |  c | c | c   c   c   c   c   c   c   c    @{}}
{\head{Group}}
 &{\head{Description}}
 &{\head{Property}}
 &{\head{imm/mut}}
 &\head{Default}&\head{Rank(D)}&\head{Size(A)}&\head{Size(D)}&\head{Cost(A)}&\head{Cost(D)}&\head{Alph(A)}&\head{Alph(D)}
 \\\hhline{============} 
\multirow{54}{*}{Linked List}  & \multirow{6}{*}{min}  & \multirow{2}{*}{AST size} & imm & 28 & 28 & 28 & 28 & 28 & 28 & 28 & 28
 \\ 
  &  &  & mut & 28 & 28 & 28 & 28 & 28 & 28 & 28 & 28
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#backtr} & imm & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2
 \\ 
  &  & & mut & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#rules} & imm & 38 & 38 & 38 & 38 & 38 & 38 & 38 & 38
 \\ 
  &  & & mut & 38 & 38 & 38 & 38 & 38 & 38 & 38 & 38
 \\ 
 \cline{2 - 12} 
 & \multirow{6}{*}{singleton}  & \multirow{2}{*}{AST size} & imm & 11 & 11 & 11 & 11 & 11 & 11 & 11 & 11
 \\ 
  &  &  & mut & 11 & 11 & 11 & 11 & 11 & 11 & 11 & 11
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#backtr} & imm & 8 & 8 & 8 & 8 & 8 & 8 & 8 & 8
 \\ 
  &  & & mut & 8 & 8 & 8 & 8 & 8 & 8 & 8 & 8
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#rules} & imm & 30 & 30 & 30 & 30 & 30 & 30 & 30 & 30
 \\ 
  &  & & mut & 30 & 30 & 30 & 30 & 30 & 30 & 30 & 30
 \\ 
 \cline{2 - 12} 
 & \multirow{6}{*}{init}  & \multirow{2}{*}{AST size} & imm & 13 & 13 & 13 & 13 & 13 & 13 & 13 & 13
 \\ 
  &  &  & mut & 13 & 13 & 13 & 13 & 13 & 13 & 13 & 13
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#backtr} & imm & 5 & 5 & 5 & 5 & 5 & 5 & 5 & 5
 \\ 
  &  & & mut & 5 & 5 & 5 & 5 & 5 & 5 & 5 & 5
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#rules} & imm & 27 & 27 & 27 & 27 & 27 & 27 & 27 & 27
 \\ 
  &  & & mut & 27 & 27 & 27 & 27 & 27 & 27 & 27 & 27
 \\ 
 \cline{2 - 12} 
 & \multirow{6}{*}{delete}  & \multirow{2}{*}{AST size} & imm & 44 & 44 & 44 & 44 & 44 & 44 & 44 & 44
 \\ 
  &  &  & mut & 44 & 44 & 44 & 44 & 44 & 44 & 44 & 44
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#backtr} & imm & 67 & 67 & 67 & 67 & 67 & 67 & 67 & 67
 \\ 
  &  & & mut & 67 & 67 & 67 & 67 & 67 & 67 & 67 & 67
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#rules} & imm & 180 & 182 & 182 & 182 & 182 & 182 & 182 & 182
 \\ 
  &  & & mut & 180 & 182 & 182 & 182 & 182 & 182 & 182 & 182
 \\ 
 \cline{2 - 12} 
 & \multirow{6}{*}{max}  & \multirow{2}{*}{AST size} & imm & 28 & 28 & 28 & 28 & 28 & 28 & 28 & 28
 \\ 
  &  &  & mut & 28 & 28 & 28 & 28 & 28 & 28 & 28 & 28
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#backtr} & imm & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2
 \\ 
  &  & & mut & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#rules} & imm & 38 & 38 & 38 & 38 & 38 & 38 & 38 & 38
 \\ 
  &  & & mut & 38 & 38 & 38 & 38 & 38 & 38 & 38 & 38
 \\ 
 \cline{2 - 12} 
 & \multirow{6}{*}{length}  & \multirow{2}{*}{AST size} & imm & 22 & 22 & 22 & 22 & 22 & 22 & 22 & 22
 \\ 
  &  &  & mut & 22 & 22 & 22 & 22 & 22 & 22 & 22 & 22
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#backtr} & imm & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2
 \\ 
  &  & & mut & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#rules} & imm & 38 & 38 & 38 & 38 & 38 & 38 & 38 & 38
 \\ 
  &  & & mut & 38 & 38 & 38 & 38 & 38 & 38 & 38 & 38
 \\ 
 \cline{2 - 12} 
 & \multirow{6}{*}{lcopy}  & \multirow{2}{*}{AST size} & imm & 32 & 32 & 32 & 32 & 32 & 32 & 32 & 32
 \\ 
  &  &  & mut & 35 & 35 & 35 & 35 & 35 & 35 & 35 & 32
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#backtr} & imm & 9 & 9 & 9 & 9 & 9 & 9 & 9 & 9
 \\ 
  &  & & mut & 14 & 24 & 24 & 24 & 24 & 24 & 24 & 13
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#rules} & imm & 66 & 66 & 66 & 66 & 66 & 66 & 66 & 66
 \\ 
  &  & & mut & 82 & 103 & 103 & 103 & 103 & 103 & 103 & 75
 \\ 
 \cline{2 - 12} 
 & \multirow{6}{*}{dispose}  & \multirow{2}{*}{AST size} & imm & 11 & 11 & 11 & 11 & 11 & 11 & 11 & 11
 \\ 
  &  &  & mut & 11 & 11 & 11 & 11 & 11 & 11 & 11 & 11
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#backtr} & imm & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0
 \\ 
  &  & & mut & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#rules} & imm & 8 & 8 & 8 & 8 & 8 & 8 & 8 & 8
 \\ 
  &  & & mut & 8 & 8 & 8 & 8 & 8 & 8 & 8 & 8
 \\ 
 \cline{2 - 12} 
 & \multirow{6}{*}{append}  & \multirow{2}{*}{AST size} & imm & 20 & 20 & 20 & 20 & 20 & 20 & 20 & 20
 \\ 
  &  &  & mut & 20 & 20 & 20 & 20 & 20 & 20 & 20 & 20
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#backtr} & imm & 8 & 8 & 8 & 8 & 8 & 8 & 8 & 8
 \\ 
  &  & & mut & 8 & 8 & 8 & 8 & 8 & 8 & 8 & 8
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#rules} & imm & 77 & 81 & 81 & 81 & 81 & 81 & 81 & 81
 \\ 
  &  & & mut & 78 & 82 & 82 & 82 & 82 & 82 & 82 & 82
 \\ 
 
 \hline 
\multirow{30}{*}{Sorted list}  & \multirow{6}{*}{ins-sort-len}  & \multirow{2}{*}{AST size} & imm & 29 & 29 & 29 & 29 & 29 & 29 & 29 & 29
 \\ 
  &  &  & mut & 29 & 29 & 29 & 29 & 29 & 29 & 29 & 29
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#backtr} & imm & 7 & 7 & 7 & 7 & 7 & 7 & 7 & 7
 \\ 
  &  & & mut & 8 & 8 & 8 & 8 & 8 & 8 & 8 & 8
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#rules} & imm & 59 & 59 & 59 & 59 & 59 & 59 & 59 & 59
 \\ 
  &  & & mut & 60 & 60 & 60 & 60 & 60 & 60 & 60 & 60
 \\ 
 \cline{2 - 12} 
 & \multirow{6}{*}{prepend}  & \multirow{2}{*}{AST size} & imm & 11 & 11 & 11 & 11 & 11 & 11 & 11 & 11
 \\ 
  &  &  & mut & 11 & 11 & 11 & 11 & 11 & 11 & 11 & 11
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#backtr} & imm & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1
 \\ 
  &  & & mut & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#rules} & imm & 17 & 17 & 17 & 17 & 17 & 17 & 17 & 17
 \\ 
  &  & & mut & 17 & 17 & 17 & 17 & 17 & 17 & 17 & 17
 \\ 
 \cline{2 - 12} 
 & \multirow{6}{*}{ins-sort-all}  & \multirow{2}{*}{AST size} & imm & 29 & 29 & 29 & 29 & 29 & 29 & 29 & 29
 \\ 
  &  &  & mut & 29 & 29 & 29 & 29 & 29 & 29 & 29 & 29
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#backtr} & imm & 5 & 5 & 5 & 5 & 5 & 5 & 5 & 5
 \\ 
  &  & & mut & 5 & 5 & 5 & 5 & 5 & 5 & 5 & 5
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#rules} & imm & 60 & 60 & 60 & 60 & 60 & 60 & 60 & 60
 \\ 
  &  & & mut & 60 & 60 & 60 & 60 & 60 & 60 & 60 & 60
 \\ 
 \cline{2 - 12} 
 & \multirow{6}{*}{insert}  & \multirow{2}{*}{AST size} & imm & 53 & 53 & 53 & 53 & 53 & 53 & 53 & 53
 \\ 
  &  &  & mut & 53 & 53 & 53 & 53 & 53 & 53 & 53 & 53
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#backtr} & imm & 35 & 34 & 34 & 34 & 34 & 34 & 34 & 34
 \\ 
  &  & & mut & 96 & 95 & 95 & 95 & 95 & 95 & 95 & 95
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#rules} & imm & 214 & 218 & 218 & 218 & 218 & 218 & 218 & 218
 \\ 
  &  & & mut & 338 & 344 & 344 & 344 & 344 & 344 & 344 & 344
 \\ 
 \cline{2 - 12} 
 & \multirow{6}{*}{ins-sort-val}  & \multirow{2}{*}{AST size} & imm & 29 & 29 & 29 & 29 & 29 & 29 & 29 & 29
 \\ 
  &  &  & mut & 29 & 29 & 29 & 29 & 29 & 29 & 29 & 29
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#backtr} & imm & 5 & 5 & 5 & 5 & 5 & 5 & 5 & 5
 \\ 
  &  & & mut & 5 & 5 & 5 & 5 & 5 & 5 & 5 & 5
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#rules} & imm & 57 & 57 & 57 & 57 & 57 & 57 & 57 & 57
 \\ 
  &  & & mut & 57 & 57 & 57 & 57 & 57 & 57 & 57 & 57
 \\ 
 
 \hline 
\multirow{84}{*}{Tree}  & \multirow{6}{*}{tcopy-ptr-all}  & \multirow{2}{*}{AST size} & imm & 46 & 46 & 46 & 46 & 46 & 46 & 46 & 46
 \\ 
  &  &  & mut & 55 & 55 & 55 & 55 & 55 & 55 & 55 & 49
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#backtr} & imm & 10 & 10 & 10 & 10 & 10 & 10 & 10 & 30
 \\ 
  &  & & mut & 88 & 88 & 88 & 88 & 88 & 88 & 88 & 168
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#rules} & imm & 93 & 93 & 93 & 93 & 93 & 93 & 93 & 152
 \\ 
  &  & & mut & 303 & 303 & 303 & 303 & 303 & 303 & 303 & 475
 \\ 
 \cline{2 - 12} 
 & \multirow{6}{*}{tcopy-all}  & \multirow{2}{*}{AST size} & imm & 42 & 42 & 42 & 42 & 42 & 42 & 42 & 42
 \\ 
  &  &  & mut & 51 & 51 & 51 & 51 & 51 & 51 & 51 & 45
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#backtr} & imm & 10 & 10 & 10 & 10 & 10 & 10 & 10 & 30
 \\ 
  &  & & mut & 88 & 88 & 88 & 88 & 88 & 88 & 88 & 168
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#rules} & imm & 85 & 85 & 85 & 85 & 85 & 85 & 85 & 144
 \\ 
  &  & & mut & 296 & 296 & 296 & 296 & 296 & 296 & 296 & 468
 \\ 
 \cline{2 - 12} 
 & \multirow{6}{*}{tsize-ptr-all}  & \multirow{2}{*}{AST size} & imm & 36 & 36 & 36 & 36 & 36 & 36 & 36 & 36
 \\ 
  &  &  & mut & 42 & 42 & 42 & 42 & 42 & 42 & 42 & 48
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#backtr} & imm & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 5
 \\ 
  &  & & mut & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 10
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#rules} & imm & 53 & 53 & 53 & 53 & 53 & 53 & 53 & 68
 \\ 
  &  & & mut & 58 & 58 & 58 & 58 & 58 & 58 & 58 & 64
 \\ 
 \cline{2 - 12} 
 & \multirow{6}{*}{tcopy-ptr-len}  & \multirow{2}{*}{AST size} & imm & 40 & 40 & 40 & 40 & 40 & 40 & 40 & 40
 \\ 
  &  &  & mut & 46 & 46 & 46 & 46 & 46 & 46 & 46 & 46
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#backtr} & imm & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 21
 \\ 
  &  & & mut & 90 & 90 & 90 & 90 & 90 & 90 & 90 & 82
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#rules} & imm & 80 & 80 & 80 & 80 & 80 & 80 & 80 & 147
 \\ 
  &  & & mut & 311 & 311 & 311 & 311 & 311 & 311 & 311 & 294
 \\ 
 \cline{2 - 12} 
 & \multirow{6}{*}{flatten-acc}  & \multirow{2}{*}{AST size} & imm & 35 & 35 & 35 & 35 & 35 & 35 & 35 & 35
 \\ 
  &  &  & mut & 35 & 35 & 35 & 35 & 35 & 35 & 35 & 35
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#backtr} & imm & 24 & 24 & 24 & 24 & 24 & 24 & 24 & 24
 \\ 
  &  & & mut & 24 & 24 & 24 & 24 & 24 & 24 & 24 & 24
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#rules} & imm & 118 & 120 & 120 & 120 & 120 & 120 & 120 & 120
 \\ 
  &  & & mut & 118 & 120 & 120 & 120 & 120 & 120 & 120 & 120
 \\ 
 \cline{2 - 12} 
 & \multirow{6}{*}{tcopy-ptr-val}  & \multirow{2}{*}{AST size} & imm & 46 & 46 & 46 & 46 & 46 & 46 & 46 & 46
 \\ 
  &  &  & mut & 55 & 55 & 55 & 55 & 55 & 55 & 55 & 49
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#backtr} & imm & 10 & 10 & 10 & 10 & 10 & 10 & 10 & 30
 \\ 
  &  & & mut & 1222 & 1222 & 1222 & 1222 & 1222 & 1222 & 1222 & 1386
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#rules} & imm & 89 & 89 & 89 & 89 & 89 & 89 & 89 & 146
 \\ 
  &  & & mut & 2679 & 2679 & 2679 & 2679 & 2679 & 2679 & 2679 & 2989
 \\ 
 \cline{2 - 12} 
 & \multirow{6}{*}{tsize-ptr-len}  & \multirow{2}{*}{AST size} & imm & 36 & 36 & 36 & 36 & 36 & 36 & 36 & 36
 \\ 
  &  &  & mut & 36 & 36 & 36 & 36 & 36 & 36 & 36 & 42
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#backtr} & imm & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 5
 \\ 
  &  & & mut & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#rules} & imm & 52 & 52 & 52 & 52 & 52 & 52 & 52 & 67
 \\ 
  &  & & mut & 53 & 53 & 53 & 53 & 53 & 53 & 53 & 53
 \\ 
 \cline{2 - 12} 
 & \multirow{6}{*}{tsize-len}  & \multirow{2}{*}{AST size} & imm & 32 & 32 & 32 & 32 & 32 & 32 & 32 & 32
 \\ 
  &  &  & mut & 32 & 32 & 32 & 32 & 32 & 32 & 32 & 38
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#backtr} & imm & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 5
 \\ 
  &  & & mut & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 2
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#rules} & imm & 44 & 44 & 44 & 44 & 44 & 44 & 44 & 59
 \\ 
  &  & & mut & 46 & 46 & 46 & 46 & 46 & 46 & 46 & 46
 \\ 
 \cline{2 - 12} 
 & \multirow{6}{*}{tcopy-len}  & \multirow{2}{*}{AST size} & imm & 36 & 36 & 36 & 36 & 36 & 36 & 36 & 36
 \\ 
  &  &  & mut & 42 & 42 & 42 & 42 & 42 & 42 & 42 & 42
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#backtr} & imm & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 21
 \\ 
  &  & & mut & 90 & 90 & 90 & 90 & 90 & 90 & 90 & 82
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#rules} & imm & 72 & 72 & 72 & 72 & 72 & 72 & 72 & 139
 \\ 
  &  & & mut & 304 & 304 & 304 & 304 & 304 & 304 & 304 & 287
 \\ 
 \cline{2 - 12} 
 & \multirow{6}{*}{tsize-all}  & \multirow{2}{*}{AST size} & imm & 32 & 32 & 32 & 32 & 32 & 32 & 32 & 32
 \\ 
  &  &  & mut & 38 & 38 & 38 & 38 & 38 & 38 & 38 & 44
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#backtr} & imm & 2 & 2 & 2 & 2 & 2 & 2 & 2 & 5
 \\ 
  &  & & mut & 4 & 4 & 4 & 4 & 4 & 4 & 4 & 10
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#rules} & imm & 45 & 45 & 45 & 45 & 45 & 45 & 45 & 60
 \\ 
  &  & & mut & 51 & 51 & 51 & 51 & 51 & 51 & 51 & 57
 \\ 
 \cline{2 - 12} 
 & \multirow{6}{*}{flatten-app}  & \multirow{2}{*}{AST size} & imm & 48 & 48 & 48 & 48 & 48 & 48 & 48 & 48
 \\ 
  &  &  & mut & 48 & 48 & 48 & 48 & 48 & 48 & 48 & 48
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#backtr} & imm & 14 & 14 & 14 & 14 & 14 & 14 & 14 & 14
 \\ 
  &  & & mut & 14 & 14 & 14 & 14 & 14 & 14 & 14 & 14
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#rules} & imm & 76 & 76 & 76 & 76 & 76 & 76 & 76 & 76
 \\ 
  &  & & mut & 76 & 76 & 76 & 76 & 76 & 76 & 76 & 76
 \\ 
 \cline{2 - 12} 
 & \multirow{6}{*}{morph}  & \multirow{2}{*}{AST size} & imm & 19 & 19 & 19 & 19 & 19 & 19 & 19 & 19
 \\ 
  &  &  & mut & 19 & 19 & 19 & 19 & 19 & 19 & 19 & 25
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#backtr} & imm & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 4
 \\ 
  &  & & mut & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#rules} & imm & 24 & 24 & 24 & 24 & 24 & 24 & 24 & 33
 \\ 
  &  & & mut & 24 & 24 & 24 & 24 & 24 & 24 & 24 & 24
 \\ 
 \cline{2 - 12} 
 & \multirow{6}{*}{dispose}  & \multirow{2}{*}{AST size} & imm & 16 & 16 & 16 & 16 & 16 & 16 & 16 & 16
 \\ 
  &  &  & mut & 16 & 16 & 16 & 16 & 16 & 16 & 16 & 16
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#backtr} & imm & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0
 \\ 
  &  & & mut & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#rules} & imm & 10 & 10 & 10 & 10 & 10 & 10 & 10 & 10
 \\ 
  &  & & mut & 10 & 10 & 10 & 10 & 10 & 10 & 10 & 10
 \\ 
 \cline{2 - 12} 
 & \multirow{6}{*}{tcopy-val}  & \multirow{2}{*}{AST size} & imm & 42 & 42 & 42 & 42 & 42 & 42 & 42 & 42
 \\ 
  &  &  & mut & 51 & 51 & 51 & 51 & 51 & 51 & 51 & 45
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#backtr} & imm & 10 & 10 & 10 & 10 & 10 & 10 & 10 & 30
 \\ 
  &  & & mut & 1222 & 1222 & 1222 & 1222 & 1222 & 1222 & 1222 & 1386
 \\ 
 \cline{3 - 12} 
 &  & \multirow{2}{*}{\#rules} & imm & 82 & 82 & 82 & 82 & 82 & 82 & 82 & 139
 \\ 
  &  & & mut & 2673 & 2673 & 2673 & 2673 & 2673 & 2673 & 2673 & 2983\\ 
 \hhline{============}  
  \end{tabular}
